Production networks and epidemic spreading: How to restart the UK economy?

We analyse the economics and epidemiology of different scenarios for a phased restart of the UK economy. Our economic model is designed to address the unique features of the COVID-19 pandemic. Social distancing measures affect both supply and demand, and input-output constraints play a key role in restricting economic output. Standard models for production functions are not adequate to model the short-term effects of lockdown. A survey of industry analysts conducted by IHS Markit allows us to evaluate which inputs for each industry are absolutely necessary for production over a two month period. Our model also includes inventory dynamics and feedback between unemployment and consumption. We demonstrate that economic outcomes are very sensitive to the choice of production function, show how supply constraints cause strong network effects, and find some counter-intuitive effects, such as that reopening only a few industries can actually lower aggregate output. Occupation-specific data and contact surveys allow us to estimate how different industries affect the transmission rate of the disease. We investigate six different re-opening scenarios, presenting our best estimates for the increase in R0 and the increase in GDP. Our results suggest that there is a reasonable compromise that yields a relatively small increase in R0 and delivers a substantial boost in economic output. This corresponds to a situation in which all non-consumer facing industries reopen, schools are open only for workers who need childcare, and everyone who can work from home continues to work from home.

==> bin.tex <==

\paragraph{Students and pupils}
We know that students and pupils are exposed to infection due to school attendance, transport, consumption, and other household interaction. We assume that pupils that go to school have the same amount of contacts in school as before lockdown\footnote{
%
We make this assumption considering that a) only certain schools are open so it is unclear to what extent the density in schools has decreased b) it is possible that pupils interact more with the few pupils left in school and thus the number of contacts can remain roughly constant.
%
}, while for transport we consider that the number of contacts decreases due to the reduced density of people in the bus/train. With these assumptions we obtain the following equation for the infection rate
\begin{eqnarray}
\frac{dS^s}{dt}  & = &  - \beta^*\Bigg[ \beta_s(0) \frac{S^s \mu^s}{\eta^s} \frac{I}{M}  +  \beta_T(0)S^s \mu^s  \left( \frac{ \mu^s \frac{I^s}{M} + \sum_{k=1}^N\delta_{k,w}\frac{I_k}{M}}{\left( \eta^s + \sum_{l=1}^N \eta_l \right)^2} \right)  \nonumber \\
 &+&\beta_c(0) S^s \frac{I}{M} \sum_{k=1}^N \delta_k(t) b_{k,c}  + \beta_h(0) S^s \frac{I}{M}  \left( (1 - \delta_h)\kappa + \delta_h \right)   \Bigg],
\end{eqnarray}
where the first two terms correspond to the infections happening at school and transport and thus only apply to the fraction $\mu^s$ of the student population that goes to school. The third and fourth term correspond to infections happening while consuming or doing other household activities and therefore apply to the whole student population. $b_{k,c}$ is the consumption related contacts, while $\kappa$  is the share of social/family/friends contacts that are not avoidable by social distancing. Notice that since transport is shared with both students and workers, the transport term includes both $I^s$ and $I_k$. The fact that we are considering the fractions $\mu^s$ and $\delta_{k,w}$ of infected in the transport term reflects our assumption that density matters in particular in transports; note, for example, that we are not multiplying infected individuals by $\mu^s$ in the school term.  The terms  $\eta^s$ and $\left( \eta^s + \sum_{l=j}^N \eta_j \right)^2$ in the denominators are normalizing factors that will be useful later. 

We simplify the above equation using the mean field approximation $S_i \approx \eta_i S$, $I_i \approx \eta_i I$, $S^s \approx  \eta^s S$, and $I^s \approx \eta^s  I$ and obtain
\begin{eqnarray}
\frac{dS^s}{dt}  & = &  - \frac{\beta^*}{M} SI\Bigg[\beta_s(0)  \mu^s   + \beta_T(0)    \left(  \frac{  (\eta^s\mu^s)^2 + \eta^s\mu^s\sum_{k=1}^N\delta_{k,w}\eta_k}{\left( \eta^s + \sum_{l=1}^N \eta_l \right)^2} \right)   \nonumber \\
 &+& \beta_c(0)\eta^s  \sum_{k=1}^N \delta_k(t) b_{k,c}  + \beta_h(0)\eta^s  \left( (1 - \delta_h)\kappa + \delta_h \right)   \Bigg]
  \label{eq:SIR_school}
\end{eqnarray}
where the normalizing factor $\eta^s$ has cancelled with the $\eta^s$ factor in $S^s$. This is important since $\beta_s(0)$ is calibrated with respect to school contacts of the total population, and thus should be multiplied by $S$ and not $S^s$.

\paragraph{Working population}
Workers are exposed to infection due to work, transport, consumption, and other household interaction. For a worker in industry $i$, the infection rate is
\begin{eqnarray}
\frac{dS_i}{dt}  & = &  -\beta^*  \Bigg[ \beta_w(0) \delta_{i,w} \frac{S_ib_{i,w}}{\sum_{l=1}^N  \eta_l b_{l,w}} \frac{I}{M}  + \beta_T(0) S_i \delta_{i,w} \left( \frac{ \mu^s \frac{I^s}{M} + \sum_{k=1}^N\delta_{k,w}\frac{I_k}{M}}{\left( \eta^s + \sum_{l=1}^N \eta_l \right)^2} \right)  \nonumber \\
 &+& \beta_c(0)S_i \frac{I}{M} \sum_{k=1}^N \delta_k(t) b_{k,c}  + \beta_h(0) S_i \frac{I}{M}  \left( (1 - \delta_h)\kappa + \delta_h \right)   \Bigg],
\end{eqnarray}
where $\sum_{l=1}^N  \eta_l b_{l,w}$ is another normalizing factor. We have assumed that workers that go to work make the same amount of contacts at work as before lockdown, while for transport we consider that the number of contacts decreases due to the reduced density of people in public transport. We have made explicit that the work and transport infection channels only apply to the fraction $\delta_{i,w}$ of the working population in $i$ going to work and to the $\mu^s$ fraction of students going to school. As before, we use the mean field approximation $S_i \approx \eta_i S$, $I_i \approx \eta_i I$, $S^s \approx  \eta^s S$, and $I^s \approx \eta^s  I$ to simplify the equation to
\begin{eqnarray}
\frac{dS_i}{dt}  & = & - \frac{\beta^*}{M} SI\Bigg[  \beta_w(0)\frac{\delta_{i,w} \eta_ib_{i,w}}{\sum_{l=1}^N  \eta_l b_{l,w}}   + \beta_T(0)\eta_i\delta_{i,w}  \left( \frac{ \mu^s \eta^s + \sum_{k=1}^N\delta_{k,w}\eta_k}{\left( \eta^s + \sum_{l=1}^N \eta_l \right)^2} \right)  \nonumber \\
 &+& \beta_c(0)\eta_i \sum_{k=1}^N \delta_k(t) b_{k,c}  + \beta_h(0) \eta_i  \left( (1 - \delta_h)\kappa + \delta_h \right)   \Bigg].
\end{eqnarray}
We now sum across all $N$ industries to obtain
\begin{eqnarray}
\sum_{i=1}^N \frac{dS_i}{dt}  & = & - \frac{\beta^*}{M} SI\Bigg[ \beta_w(0) \sum_{i=1}^N\delta_{i,w}\frac{ \eta_ib_{i,w}}{\sum_{l=1}^N \eta_l b_{l,w}}  + \beta_T(0) \left( \frac{ \mu^s \eta^s \sum_{i=1}^N \eta_i\delta_{i,w} + \left(\sum_{i=1}^N \eta_i\delta_{i,w}\right)^2 }{\left( \eta^s + \sum_{l=1}^N \eta_l \right)^2} \right)  \nonumber \\
 &+& \beta_c(0)\sum_{i=1}^N \eta_i \sum_{k=1}^N \delta_k(t) b_{k,c}  +\beta_h(0) \sum_{i=1}^N \eta_i  \left( (1 - \delta_h)\kappa + \delta_h \right)   \Bigg].
  \label{eq:SIR_work}
\end{eqnarray}

\paragraph{Non-working adults}
By definition non-working adults are not exposed to the work or school infection channel. Furthermore, since we only consider work-commuting transport use, the non-working adults are not exposed to the transport infection channel either. It follows that the decrease in the susceptible population depends only on the consumption and other household interaction channel
\begin{equation}
    \frac{dS^u}{dt} = - \frac{\beta^*}{M} S I \Big[ \beta_c(0) \eta^u \sum_{k=1}^N \delta_{k,c}(t)  b_{k,c} + \beta_h(0) \eta^u \left( (1 - \delta_h)\kappa + \delta_h \right),  
    \Big]
    \label{eq:SIR_nonworking}
\end{equation}
where we have again used the approximation  $S^u \approx \eta^u S$.
%where we have assumed homogenous mixing of the population, meaning that the probability that a person an individual had contact with was infected is $\frac{I}{M}$. %$b_{k,c}$ and $b_h$ are the consumption and other household interaction related contacts, while $\kappa$  is the share of social/family/friends contacts that are not avoidable by social distancing. 
% We can further simplify the above equation into
% \begin{equation}
%     \frac{dS^u}{dt} = - \frac{\beta^*}{M} S^u I \Big[ \underbrace{  \sum_{k=1}^N \delta_{k,c}(t)  b_{k,c}}_\textrm{consumption} + \underbrace{b_h \left( (1 - \delta_h)\kappa + \delta_h \right) }_\textrm{other}  
%     \Big]
%     \label{eq:SIR_nonworking}
% \end{equation}
\paragraph{Total population}
To get the infection rate of the overall population we substitute Eqs. \ref{eq:SIR_school}--\ref{eq:SIR_nonworking} in equation Eq. \ref{eq:SIR_allapx}. It follows that 
\begin{eqnarray}
\frac{dS}{dt}  & = &  - \beta^* \frac{SI}{M}\Bigg[ \beta_w(0) \sum_{i=1}^N\delta_{i,w}\frac{ \eta_ib_{i,w}}{\sum_{l=1}^N \eta_l b_{l,w}} + \beta_s(0)  \mu^s \nonumber \\
 &+& \beta_T(0) \left( \frac{ \mu^s \eta^s +\sum_{i=1}^N \eta_i\delta_{i,w} }{\eta^s + \sum_{l=1}^N \eta_l} \right)^2  \nonumber \\
 &+& \beta_c(0) \sum_{k=1}^N \delta_k(t) b_{k,c}  +  \beta_h(0)  \left( (1 - \delta_h)\kappa + \delta_h \right)   \Bigg],
\end{eqnarray}
where we have used the fact that $ \eta^s + \eta^u + \sum_{i=1}^N \eta_i = 1.$ The above terms correspond to the infection due to work, school, transport, consumption, and other household interaction respectively. We can write the above equation as
\begin{equation}
 \frac{dS}{dt}  = - \beta(t)\frac{SI}{M}
\end{equation}
where 
\begin{equation}
   \beta(t) = \beta^* \Big( \beta_w(t)+\beta_s(t)+\beta_c(t)+\beta_T(t)+\beta_h(t) \Big),
\end{equation}
which is Eq.\ref{eq:beta} of the main text. The $\beta$'s are given by
\begin{equation}
   \beta_w(t) =   \beta_w(0) \sum_{i=1}^N\delta_{i,w}\frac{ \eta_ib_{i,w}}{\sum_{l=1}^N \eta_l b_{l,w}}
\end{equation}
\begin{equation}
   \beta_s(t) =  \beta_s(0)   \mu^s,
\end{equation}
\begin{equation}
   \beta_T(t) = \beta_T(0) \left( \frac{  \mu^s \eta^s +\sum_{i=1}^N \eta_i\delta_{i,w} }{\eta^s + \sum_{l=1}^N \eta_l} \right)^2 
\end{equation}
\begin{equation}
   \beta_c(t) =   \beta_c(0) \sum_{k=1}^N \delta_k(t) b_{k,c},
\end{equation}
and
\begin{equation}
   \beta_h =   \beta_h(0)  \left( (1 - \delta_h)\kappa + \delta_h \right).
\end{equation}
The normalizing factors guarantee that at the time before lockdown all the above equations are consistent. %To obtain the definition expressed in the main text for all $\beta$'s we  substitute the definition $\mu^s$. This step completes the derivation.











% \MdRC{To update to proper SEIAHR}
%We now focus on the contribution of each activity to the rate of infection. Let $S_i$, $I_i$, and $R_i$ denote the number of susceptible, infected and recovered workers form industry $i$. The rate at which susceptible workers of industry $i$ get infected is the sum of the rates of infection due to work, consumption, transport and other household interactions
%\begin{equation}
%    \frac{dS_i}{dt} = - \frac{\beta_0}{N} \Big[ \underbrace{ b_w S_iI  \delta_{iw}(t) \frac{b_{i,w}}{\mathcal{N}_b}}_\textrm{work} +  \underbrace{b_c S_i I  \sum_{k=1}^M \delta_{kc}(t) b_{k,c}}_\textrm{consumption} + \underbrace{b_{T} S_i \delta_{iw}(t)  \sum_{k=1}^M\delta_{kw}(t)I_k}_\textrm{transport} + \underbrace{b_h \kappa(t) S_i   I}_\textrm{other}  
%    \Big]
 %   \label{eq:SIR_i1}
%\end{equation}
%where $\beta_0$ is the baseline infection rate and the $b_w, b_c, b_t$ and $b_h$ terms account for the fraction of contacts that happen within each activity. %and $\mathcal{N}_b$ is a normalizing factor given by
% \begin{equation}
%   \mathcal{N}_w = \sum_{i=1}^M n_i  b_{i,w},
% \end{equation}
% which corresponds to the total fraction of work contacts when all industries are open.
%Note that the transport term differs from the others in that it includes a product of $\delta_{iw}$ times a sum of $\delta_{kw}$ over the open industries.  This is because the open industries increase the number of people in the transport system and correspondingly increase the likelihood of infection for a worker from industry $i$.  
%If we assume the fraction of workers who are susceptible or infected is then same in each industry (this is a mean field approximation), then $S_i = n_i S$ and $I_i = n_iI$, and we can rewrite this as 
%\begin{equation}
 %   \frac{dS_i}{dt} = - \frac{\beta_0}{N} SI\Big[  b_w\delta_{iw} n_i \frac{b_{i,w}}{\mathcal{N}_b} + 
%    b_c n_i \sum_{k=1}^M \delta_k(t) b_{k,c} + b_{T} n_i\delta_{iw} \sum_{k=1}^M\delta_{kw}(t)n_k + b_h n_i  \kappa(t)
 %   \Big]
  %  \label{eq:SIR_i2}
%\end{equation}
%We now sum across all $M$ industries and use $\sum_i n_i = 1$, to obtain the rate of infection of the overall population
%\begin{equation}
%     \frac{dS}{dt} = - \frac{\beta_0}{N} SI\Big[ b_w \sum_{i=1}^M \delta_{iw}(t) n_i\frac{b_{i,w}}{\mathcal{N}_b} + 
%     b_c \sum_{k=1}^M \delta_{kc}(t) b_{k,c} + b_{T} \sum_{i=1}^M\delta_{iw}(t) n_i\sum_{k=1}^M\delta_{kw}(t)n_k +  b_h \kappa(t)
%     \label{eq:SIR_i3}
%    \Big]
%\end{equation}



We indicate whether an industry $i$ is open or closed for work by $\delta_{i,w}(t)$  where
\begin{equation}
    \delta_{i,w}(t)  = 
        \begin{cases}
      1 & \text{if}\ \text{industry} ~i \text{ is open for work at time } t \\
      0 &  \text{otherwise}. \\
    \end{cases}
\end{equation} 
If an industry is closed then people cannot go to work and stay at home. Similarly, we indicate  whether an industry $i$ is open or closed for on-site consumption by $\delta_{ic}(t)$  where
\begin{equation}\label{eq:onsiteconsumption}
    \delta_{i,c}(t)  = 
        \begin{cases}
      1 & \text{if}\ \text{industry} ~i \text{ is open for on-site consumption at time } t \\
      0 &  \text{otherwise}. \\
    \end{cases}
\end{equation} 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The contacts an average person has are split among the different activities work, consumption, transport and other. We denote the fraction of contacts happening during each activity by $b_w$, $b_c$, $b_T$, and $b_h$, where $b_w + b_c + b_T + b_h = 1$.

We account for the heterogeneity of contacts that happen at work and during consumption within different industries. For example, most industries do not receive customers and therefore do not account for any of the consumption contacts. We denote the fraction of the fraction of all consumption contacts that happen within industry $i$ by $b_{ic}$, where $\sum_i b_{ic} = 1$. As we discuss later in the calibration section, only three industries have non-negligible contribution to consumption contacts (retail, hospitality, and entertainment).

For the work scenario we take a slightly different approach. Since the nature of work varies across industries we denote the relative contact risk a workers of industry $i$ faces by $b_iw$, where $\sum_i b_{iw} = 1$. This means that if $b_{iw} = 2b_{jw}$ a worker of industry $i$ is twice as exposed to the virus than a workers in industry $j$. The fraction of all the work contacts an industry $i$ accounts for is 
$$ \frac{n_i b_{iw}}{\sum_k n_k b_{kw}}.$$
For the derivations we do later it is convenient to define the normalizing factor
\begin{equation}
    \mathcal{N}_w = \sum_k n_k b_{kw}.
\end{equation}{}

Finally, we assume that people only use transport to go to work and that due to social distancing regulations household interactions are reduced up to a $\kappa(t)$ fraction. 

%%%%%%%%%%%%%%%%%%%%%%%%%%



\MdRC{Instead of having $\delta(t)$ I think it makes more sense to have $\delta(scenario)$.}

A full policy scenario $\sigma$ is the combination of a consumption policy scenario and a work policy scenario, i.e. $\sigma = (\sigma_w, \sigma_c).$ 

We consider different work and consumption policies, where work policies determine how many workers from each industry can work and consumption policies determine which industries are open for on-site consumption. We denote a work policy scenarios by $\sigma_w$, and the fraction of workers of industry $i$ that go to work within that policy by $\delta_{iw}(\sigma_w)$. Similarly, $\sigma_c$ denotes a consumption policy, and the amount of on-site consumption allowed in the industry $i$ by $\delta_{ic}(\sigma_c)$. 

\paragraph{Consumption policies.} We consider two policy scenarios for consumption

$\sigma_c \in \left\{\text{All open}, \text{Essential only} \right\}$ determined as follows
\begin{itemize}
    \item \textbf{All open.} All industries are allowed to receive customers on-site, i.e.    $$\delta_{ic}(\text{All open}) = 1 \ \forall i$$
    \item \textbf{Essential only.} Only essential good selling industries (e.g. grocery stores) are allowed to receive customers on-site, i.e.  $$\delta_{ic}(\text{Essential only}) = e_{ic}  \ \forall i,$$ where $e_{ic}$ denotes the fraction of ``stores" that sell essential goods within the industry. 
\end{itemize}


\paragraph{Work policies.}
We consider five policy scenarios for work. In all work scenarios, except for the pre-lockdown scenario, we assume that all workers that can work remotely do not go to work.  For the lockdown and after lockdown scenarios we assume that all essential workers that need to go to work are still allowed to go to work. We denote the fraction of workers of an industry that can work remotely by $r_i$ and the fraction of essential workers of an industry by $e_{iw}$. We interpret these fractions as probabilities: the probability that a worker of industry $i$ can work remotely and the probability that a worker from industry $i$ has an essential job, we assume independence between the two.

Most schools have been closed, but some are still open for the kids of a parent(s) that have an essential job that cannot be done remotely. For the number of people attending the special $i = school$ industry we deal as follows. We assume that all $14$ years-old or younger kids need childcare, and let by $g$ denote the fraction of people (kids) in the special $i = school$ industry that are below $14$ years-old or younger. (In other words $g n_{school}$ is the fraction of the population  that are below $14$ years-old or younger). We assume the fraction of people attending school is
$$
g \times n_{school} \times  w(\sigma_w),
$$
where $w(\sigma_w)$ is the fraction of the population 20 years-old or older that is working i.e. the potential parents that may require childcare services. The fraction of the population 20 years old or older is $1 - n_{school}$ (we use this later).

\MdRC{I had to add the $14$ yo threshold because we assume that everyone between 0-19 years old is going to school so $n_{school} = 23\%$ of the population. It seemed unrealistic to have 19 year old going to school because their parent(s) were at work. I can cut the threshold at $9$ or $14$, the latter seemed better? I can also remove it by doing $g=1$}

The work policy scenarios we consider are

$\sigma \in \left\{\text{All Open}, \text{Essential only},\text{Open A-F}, \text{Open all but consumer-facing}, \text{Close Ent.},  \right\}, $ as follows,


\MdRC{I removed Open A-C since dif with A-F is marginal.}
\begin{itemize}
    \item \textbf{Pre-lockdown.} All workers of all industries go to work
    $$\delta_{iw}(\text{All open}) = 1 \ \forall i$$
    \item \textbf{Essential only.} Only essential workers that cannot go to work from home go to work.
    \begin{equation}
        \delta_{iw}(\text{Essential only})  = 
            \begin{cases}
          e_{iw}(1 - r_i) & \quad \forall i \neq school\\
         g n_{school}w(\text{Essential only}) &  \quad i = school,\\
        \end{cases}
        \nonumber
        \end{equation} 
    where 
    $$w(\text{Essential only}) = \frac{\sum_{i \neq {school}} e_{iw}(1 - r_i)n_i}{1 - n_{school}} $$

    \item \textbf{Open A-F} Essential and Non-essential workers that cannot work from home of industries A-C (Food, mining, and manufacturing, ... Construction) go to work. For all other industries only essential workers that cannot go to work from home go to work.
      \begin{equation}
        \delta_{iw}(\text{Open A-F})  = 
            \begin{cases}
          (1 - r_i) & \quad \forall i \in \text{A-F}. \\
          e_{iw}(1 - r_i) &  \quad \forall i  \notin \text{A-f}\cup school.\\
          g n_{school}w(\text{Open A-F}) & \quad  i = school.\\
        \end{cases}
        \nonumber
        \end{equation} 
       $$w(\text{Open A-C}) = \frac{\sum_{i \neq {school, A-F}} e_{iw}(1 - r_i)n_i + \sum_{i= A,...,F} (1 - r_i)n_i}{1 - n_{school}} $$    
        
    \item \textbf{Close Ent. \& Sch.} Essential and Non-essential workers that cannot work from home of all industries go to work, except for the workers in the entertainment industries (G-17, I, R\_S). For all other industries only essential workers that cannot go to work from home go to work.
      \begin{equation}
        \delta_{iw}(\text{Close Ent. \& Sch.})  = 
            \begin{cases}
          (1 - r_i) & \forall i \notin \text{G17, R\_S, I}. \\
          e_{iw}(1 - r_i) &  \forall i  \in \text{G17, R\_S, I}\\
          g n_{school}w(\text{Close Ent. \& Sch.}) &  i = school.\\
        \end{cases}
        \nonumber
        \end{equation} 
    \MdRC{todo: add here $w()$ or this of a better way to parse this (brain dead now) }  
     \item \textbf{Open Schools} Essential and Non-essential workers that cannot work from home of all industries go to work, except for the workers in the entertainment industries (G-17, I, R\_S). For all other industries only essential workers that cannot go to work from home go to work. Schools are open so they receive all students.
      \begin{equation}
        \delta_{iw}(\text{Close Ent.})  = 
            \begin{cases}
          (1 - r_i) & \quad \forall i \notin \text{G17, R\_S, I}. \\
          e_{iw}(1 - r_i) &  \quad \forall i  \in \text{G17, R\_S, I}\\
          n_{school} & \quad  i = school.\\
        \end{cases}
        \nonumber
        \end{equation} 
    % \item \textbf{Close entertainment} Essential and Non-essential workers that cannot work from home of all industries go to work, except for the workers in the entertainment industries (G-17, I, R\_S). For all other industries only essential workers that cannot go to work from home go to work. Schools are open so they receive all students.
    %   \begin{equation}
    %     \delta_{iw}(\text{Close Ent.})  = 
    %         \begin{cases}
    %       (1 - r_i) & \quad \forall i \notin \text{G17, R\_S, I}. \\
    %       e_{iw}(1 - r_i) &  \quad \forall i  \in \text{G17, R\_S, I}\\
    %       n_{school} & \quad  i = school.\\
    %     \end{cases}
    %     \nonumber
    %     \end{equation} 
\end{itemize}

\MdRC{Caveat: Note that workers in education, air and land transport are still going to work. Particularly for transport they are essential and have low remote labor index, this is unrealistic. We can try and fix it similar to schools. Open proportional to $w(\sigma_w)$, might be work for later version though.}  

\paragraph{Policy scenarios}
A full policy scenario $\sigma$ is the combination of a consumption policy scenario and a work policy scenario, i.e. $\sigma = (\sigma_w, \sigma_c).$ We list the full policy scenarios we consider below.

\begin{table}[htbp]
	\centering
	\caption{Policy scenarios }
		\begin{tabular}{c|c|c}
			 Policy $\sigma$ & Consumption side $\sigma_c$ & Work side $\sigma_w$ \\
			 	\hline
			 Pre-lockdown & All Open & All Open \\
			 Lockdown & Essential only & Essential only \\
			 Open A-C & Essential only &Open A-C \\
			 Open A-F & Essential only &Open A-F \\
			 Close Ent. \& Sch. & Essential only & Close Ent. \& Sch. \\
			 Close Ent. & Essential only & Close Ent. \\
			 %Work from home & All Open & All Open (but work from home) \\
								
		\end{tabular}
	\label{tab:scenarios}
\end{table}


In all scenarios, we apply except ``Reopen as normal'', we apply these two principles:
\begin{itemize}
    \item Work from home if you can
    \item If unemployed, furloughed, or \FL{able to work from home (?)}, keep children home
\end{itemize}





\begin{table}[H]
\centering
\begin{tabular}{r|r|r|r}
Parameter & Name & Value & Sources\\ 
  \hline
$R_0$ & Basic reproduction number & 2.6, & \\ 
$R_0$ std & Basic reproduction number & 0.54, &\\ 
  $\gamma$ & Recovery rate\footnote{
  %
  7 days is the time it takes for a person to either recover or self-isolate/go to a hospital.
  %
  }
  & 1/7 days& \cite{arenas2020mathematical}\\ 
  $\beta_0 $ & effective transmission rate & 0.38&  $R_0 \gamma$ \\ 
\end{tabular}
\label{table:sharesall}
\end{table}
 
 We estimate the percentage of kids attending school as follows. Based on the remote labor index and essential score of industries 
% According to the ONS Labour Force Survey, \footnote{
% %
% https://www.ons.gov.uk/employmentandlabourmarket/peopleinwork/employmentandemployeetypes/articles/familiesandthelabourmarketengland/2019
% %
% }
% $p_w = 75.1\%$ and $p_m = 92.6\%$ of mother and father with dependent children were in work in the UK respectively. We assume that each kid has one mother and one father. Therefore, the probability





%%%%
School stuff


%$$
%\delta_{\text{school},w}(\Lambda) = g \times \eta_{\text{school}} \times  %\frac{\sum_{i \in {\text{Open industry}}} %\delta_{i,w}(\Lambda)\eta_i}{1 - \eta_{\text{school}} }  ,
%$$
%where $w(\Lambda)$ is the fraction of the population 20 years-old or older that is working in a given scenario $\Lambda$, i.e. the potential parents that may require childcare services. The fraction of the population 20 years old or older is $1 - n_{school}$. Thus, we have
%\[
%w(\Lambda) = \frac{\sum_{i \in {\text{Open industry}}} %\delta_{i,w}(\Lambda)\eta_i}{1 - \eta_{\text{school}} }  
%\]

%We estimate the fraction children who require school services as follows. First we assume that only children below 14 year old need to go to school if parents are working. Second, 
%Assume that all $14$ years-old or younger need childcare, and let $g$ denote the fraction of children who $14$ years-old or younger. (In other words $g \eta_{school}$ is the fraction of the population that are $14$ years-old or younger). The fraction of people attending school depends on the scenario, and is computed by

%%%%%%


%\footnote{$R_0$ is well defined for the beginning of an epidemic. After one should consider $R_t = \frac{S(t)}{N}R_0.$ However, under the approximation $\frac{S}{N} \approx 1$, and because the precise number of susceptible people is unknown,  we choose to focus on $R_0$. Recently estimated attack rates for the worse affected region of Italy (Lombardy) are 13\% \citep{vollmer2020}.}
%and as result providing good epidemiological forecasts should be based on simulations where the time path of all parameters can be taken into account. In this paper, we simply use 


==> executive_summary.tex <==
\newpage
\section*{Executive summary} 
\label{sec:summary}

We evaluate the costs and benefits of reopening different parts of the economy. We consider the cost (in terms of infection risk) of reopening industries (workers and consumers get infected), and the benefit (in terms of economic output) of reopening industries (Direct and indirect output from opening the industry, where indirect effects arise because of the interdependencies between industries.)

There is considerable uncertainty in all the numbers that we have been able to find or derive, but one conclusion appears robust: 

\vspace{5mm}
\noindent
\textbf{A large part of the ``upstream'' economy that is currently closed tends to have a relatively low risk for workers, little risk for consumers, and also has high economic value.}
\vspace{5mm}

Essentially, this is because large parts of manufacturing and business services have high value added and are ``upstream'' (provide inputs to other industries); these industries are also rarely selling directly to consumers, and thus present limited risks in their contribution to the pandemic.


\paragraph{Does contamination take place mostly at work?} We find that workplace contagion is a major contributor. In our estimates, work (including schools) is responsible for 57\% of infections (with work and schools being responsible for roughly half each), consumption (retail, restaurants and entertainment) is responsible for 16\%, transport for 6\%, and household or socially-related infections represent 21\%. In comparison, the Imperial study \citep{ferguson2020} assumes that ``approximately one third of transmission occurs in the household, one third in schools and workplaces and the remaining third in the community'', so we believe that if anything, we overestimate the risk of work-related transmission.


\paragraph{Do industries/occupation vary widely in the risk for workers?} Yes, some occupations are much safer than others in normal times, and some are much easier to perform at home. We use data on occupation-specific infection risk and ability to work from home to evaluate this.


\paragraph{Do industries pose a risk for consumers?} We estimate that consumption is responsible for 16\% of all infections. However, only very few industries are consumer-facing. We think the vast majority of consumption-related infections are in the hospitality industry (23\%), in entertainment (52\%), and in retail (25\%). There is significant uncertainty and a lot of heterogeneity between specific consumption activity that we cannot evaluate with current data.


\paragraph{Is it possible to reopen only some industries?} Some industries are much more systemic than others, in the sense that they provide inputs to other industries that in turn provide inputs to other industries. As a result, it is important to reopen enough industries ``upstream'' so that industries ``downstream'' can function.
%even if they are open. 
Manufacturing and business services tend to be upstream. Personal services and retail are downstream. In our simulations, we find that reopening only very small parts of the economy causes coordination problems in supply chains, so that there is at best only a limited boost to economic output.  Thus in our scenarios we open large parts of the economy in blocks. 

\paragraph{Five re-opening scenarios}
We estimate that currently $37\%$ of workers are going to work physically (those workers that are essential and cannot work from home) and these workers are responsible for about half of the remaining infections taking place at the moment (non-work-related infection is the other half).

We propose 5 re-opening scenarios in Table \ref{table:scenario_summary_excsummary}. In all but the pre-lockdown scenario we assume that the 44\% of workers who can work from home continue to do so. We assume that schools remain partially open, that is, open only for children of parents who have to go to work physically (are employed in a reopened industry and cannot work from home). The scenarios then depend on which industries are opened.
%only Agriculture, Manufacturing, Mining and Construction (\emph{I: Manufacturing}); adding also all non consumer-facing industries (\emph{II and III: Intermediates}, because these are intermediate goods and services); and opening all industries (\emph{V: Open})


\begin{table}[H]
\footnotesize
\centering
\begin{tabular}{|p{4.4cm}|p{1.4cm}|p{1.9cm}|p{1.8cm}|p{1.8cm}|p{1cm}|p{1.4cm}|}
\hline
 & I & II & III & IV & V & VI\\
\hline
\textbf{Scenario} & Lockdown & Manufacturing and Construction & All except consumer-facing & All except consumer-facing, Schools opened & Open & Pre-lockdown\\
  \hline
\textbf{Work from home?} & Yes & Yes &Yes & Yes & Yes & No\\
\hline
\textbf{Schools open?} & Partially  & Partially  & Partially &  Fully &  Fully & Fully \\ 
\hline
\textbf{On-site consumption open?} &No &No &No &  No & Yes & Yes \\ 
 \hline
\end{tabular}
\caption{Six scenarios for reopening the economy.  {\it Lockdown} corresponds to the present situation.  {\it Manufacturing and Construction} opens these industries.  {\it All except consumer-facing} corresponds to all non-consumer facing industries, that is most services.  {\it All except consumer-facing, Schools opened} corresponds to opening schools as well.  {\it Open} corresponds to opening everything.  {\it Pre-lockdown} is listed as a separate category because in this case people do not work from home.
}
\label{table:scenario_summary_excsummary}
\end{table}
\normalsize


The results of the scenarios are in Fig. \ref{fig:scenarios}. The message is that reopening all the non-consumer-facing industries provides a large economic boost with a limited increase in infections. It remains difficult to know whether opening these industries makes $R_0>1$ or not, but we can say that they provide the highest ``bang-for-the-buck'', because they are upstream and they do not contribute to consumer-related infections.

\begin{figure}%[H]
    \centering
\includegraphics[width = 1.0\textwidth]{fig/scenarios_overlap_ratio_rescalerR0.png}
    \caption{\textbf{How different policy scenarios affect $R_0$ and economic output.} The coloured bars show the expected reproduction number of the epidemic for each policy scenario. Different colours designate the activities that cause the epidemic to spread. The purple bars denote the percentage increase in value added relative to lockdown a month after the economy is opened under each scenario.  Black lines are two standard deviation error bars. {\it Note that we have normalized the infection rates for all scenarios so that they correspond to the \cite{jarvis2020quantifying} study during lockdown.} (Our estimate during lockdown is roughly $R_0 = 0.99$; their estimate is $0.62$; these agree with the error bars).  Note that Manufacturing and Construction also includes mining, agriculture, and a few others.}
        \label{fig:scenarios}
\end{figure}

{\bf We should close by stressing that there are large uncertainties in all of our estimates.}


\newpage

